Anytime MiniBatch: Exploiting Stragglers in Online Distributed Optimization

Distributed optimization is vital in solving large-scale machine learning problems. A widely-shared feature of distributed optimization techniques is the requirement that all nodes complete their assigned tasks in each computational epoch before the system can proceed to the next epoch. In such settings, slow nodes, called stragglers, can greatly slow progress. To mitigate the impact of stragglers, we propose an online distributed optimization method called Anytime Minibatch. In this approach, all nodes are given a fixed time to compute the gradients of as many data samples as possible. The result is a variable per-node minibatch size. Workers then get a fixed communication time to average their minibatch gradients via several rounds of consensus, which are then used to update primal variables via dual averaging. Anytime Minibatch prevents stragglers from holding up the system without wasting the work that stragglers can complete. We present a convergence analysis and analyze the wall time performance. Our numerical results show that our approach is up to 1.5 times faster in Amazon EC2 and it is up to five times faster when there is greater variability in compute node performance.

==> derivations.tex <==
\section{Proof of Thm.~\ref{thm.samplePath}}
\label{sec.pfThmSampPath}


\section{Proof of Cor.~\ref{cor.samplePath}}
\label{sec.pfCorSampPath}

\section{Proof of Thm.~\ref{thm.expWork}}
\label{sec.pfThmExpWork}


\section{Proof of Cor.~\ref{cor.expWork}}
\label{sec.pfCorExpWork}

\section{Proof of Thm.~\ref{thm.speedUp}}
\label{sec.pfThmSpeedUp}




	\subsection{Appendix A}
		
	Let $z(t+1)$ be the exact dual variable without any consensus errors for each node, i.e., $z(t+1)=\bar{z}(t)+g(t)$. We bound the error due to limited consensus
	\begin{equation}
	\|z_i(t)-z(t)\| \leq \epsilon, \;\; \forall v, t.
	\end{equation} 
	Let $w(t+1)$ be the primal variable computed using $z(t+1)$:
	\begin{align}
	\label{eqn:correct.w}
	w(t+1) = \arg \min_{w \in W} \{\langle w,z(t+1)\rangle+\beta(t+1) h(w)\}
	\end{align} 
	From \cite{}[Lemma 2, need citation], we have
	\begin{align}
	\|w_i(t)-w(t)\| &\leq \frac{1}{\beta(t)} \|z_i(t)-z(t)\| \\ & \label{eqn:primary.bound}\leq \frac{\epsilon}{\beta(t)}.
	\end{align}
	
	
	We add and subtract $F(w(t))$ from \eqref{eqn:first.regret}
	\begin{align}
	\mathbb E[R]&= \mathbb E\left[\sum_{t=1}^{\tau} \sum_{i=1}^{n} \sum_{s=1}^{c_i(t)} F(w(t))-F(w^*) + F(w_i(t)) - F(w(t))\right] \\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)] + \sum_{t=1}^{\tau} \sum_{i=1}^{n} c_i(t) [F(w_i(t)) - F(w(t))]\right]
	\\ & \leq \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)] + \sum_{t=1}^{\tau} \sum_{i=1}^{n} c_i(t) L\|w_i(t)) - w(t)\|\right]
	\\ & \leq \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)] + \sum_{t=1}^{\tau} \sum_{i=1}^{n} \frac{c_i(t) L\epsilon} {\beta( t)}\right]
	\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + L\epsilon \sum_{t=1}^{\tau} \frac{c(t)} {\beta( t)}\label{eqn:regret.first}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	Now, we bound the first term. Note that $g(t)$ is calculated with respect to $w_i(t)$ by different nodes in \eqref{eqn:mini.batch}. Let $\bar g(t)$ be the mini-batch calculated with respect to $w(t)$ (given in \eqref{eqn:correct.w}) by all the workers. 
	\begin{equation}
	\label{eqn:exact.mini.batch}
	\bar g(t) =\frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w f(w(t),x_i(t,s)).
	\end{equation}
	Note that there are two types of errors in computing gradients. The first one is typical in any sub-gradient methods. That is, the gradient is calculated with respect to the function $f(w,x)$ using the data $x$ instead of directly evaluating $\nabla_w F(w)$. We denote this error as $q(t)$:
	\begin{align}
	\label{eqn.q}
	q(t) = \bar g(t)-\nabla_w F(w(t)).
	\end{align}
	The second error is we use $g(t)$ instead of $\bar g(t)$ and this error is we denote using $r(t)$:
	\begin{align}
	\label{eqn.r}
	r(t) = g(t)-\bar g(t).
	\end{align}
	{\lemma The following holds
		\begin{align}
		\mathbb E[\langle q(t),w^*-w(t)\rangle] =0,
		\end{align}
		\begin{align}
		\mathbb E[\langle r(t),w^*-w(t)\rangle] =\frac{K D \epsilon}{\beta(t)},
		\end{align}
		\begin{align}
		\mathbb E[\|q(t)\|^2]= \frac{\sigma^2}{b(t)},
		\end{align}
		\begin{align}
		\mathbb E[\|r(t)\|^2]= \frac{K^2\epsilon^2}{\beta(t)^2}.
		\end{align}}
	Proof of Lemma 6 is given in the Appendix B. Let $l_t(w)$ be the first order approximation of $F(w)$ at $w(t)$
	\begin{align}
	\label{eqn.lt}
	l_t(w)=F(w(t))+\langle \nabla_w F(w(t)),w-w(t)\rangle.
	\end{align}
	Let $\tilde l_t(w)$ be an approximation of $l_t(w)$ by replacing $\nabla_w F(w(t))$ by $g(t)$
	\begin{align}\label{eqn:approx.first.order}
	\tilde l_t(w)&=F(w(t))+\langle g(t),w-w(t)\rangle\\&=\label{eqn:approx.first.order.2}F(w(t))+\langle \nabla_w F(w(t)),w-w(t)\rangle +\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle\\&=l_t(w) +\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle\label{eqn:approx.first.order.3}
	\end{align}
	Note that \eqref{eqn:approx.first.order.2} is due to $g(t)=q(t)+r(t)+\nabla_w F(w(t))$ from \eqref{eqn.q} and \eqref{eqn.r}.  
	By using the smoothness property of $F(w)$, we can write 
	\begin{align}
	F(w(t+1)) &\leq l_t(w(t+1))+\frac{K}{2}\|w(t+1)-w(t)\|^2\\&=\tilde l_t(w(t+1))-\langle q(t),w-w(t)\rangle-\langle r(t),w-w(t)\rangle+\frac{K}{2}\|w(t+1)-w(t)\|^2
	\\&=\tilde l_t(w)+\| q(t)\|\|w-w(t)\|+ \|r(t)\|\|w-w(t)\|+\frac{K}{2}\|w(t+1)-w(t)\|^2\label{eqn.temp.fw}	
	\end{align}
	The last step is due to Cauchy-Schwarz. Let $\alpha(t)=\beta(t)-K$. We add and subtract $\alpha (t)\|w(t+1)-w(t)\|^2/2$ to find 
	\begin{align}
	F(w(t+1)) &\leq \tilde l_t(w(t+1))+\| q(t)\|\|w-w(t)\|-\frac{\alpha(t)}{4}\|w(t+1)-w(t)\|^2+ \|r(t)\|\|w-w(t)\|\\&-\frac{\alpha(t)}{4}\|w(t+1)-w(t)\|^2+\frac{K+\alpha(t)}{2}\|w(t+1)-w(t)\|^2
	\end{align}
	Note that 
	\begin{align}
	&\| q(t)\|\|w-w(t)\|-\frac{\alpha(t)}{4}\|w(t+1)-w(t)\|^2 \\&= \frac{\|q(t)\|^2}{4\alpha(t)} - \left[\frac{\|q(t)\|}{\sqrt{4\alpha(t)}} - \sqrt{\frac{a(t)}{4}} \|w(t+1)-w(t)\| \right]^2\\& \leq \frac{\|q(t)\|^2}{4\alpha(t)} \label{eqn.bound.q}
	\end{align}
	Similarly, we have
	\begin{align}
	\| r(t)\|\|w-w(t)\|-\frac{\alpha(t)}{4}\|w(t+1)-w(t)\|^2 \leq \frac{\|r(t)\|^2}{4\alpha(t)} \label{eqn.bound.r}
	\end{align}
	Using \eqref{eqn.bound.q}, \eqref{eqn.bound.r}, and $\beta(t)=K+\alpha(t)$ in \eqref{eqn.temp.fw} we have
	\begin{align}
	F(w(t+1)) \leq \tilde l_t(w(t+1))+\frac{\beta(t)}{2}\|w(t+1)-w(t)\|^2+\frac{\|q(t)\|^2}{4\alpha(t)}+\frac{\|r(t)\|^2}{4\alpha(t)}\label{eqn:bound2}
	\end{align}
	By using \cite{}[Lemma 6, need citation], we have
	\begin{align}
	\frac{\beta(t)}{2} \|w(t+1)-w(t)\|^2 &\leq \sum_{t'=1}^{t-1}\tilde l_{t'}(w(t+1))+(\beta(t))h(w(t+1))\nonumber \\ &-\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+(K+\beta(t))h(w(t))\label{eqn:bound1}
	\end{align}
	Use \eqref{eqn:bound2} in \eqref{eqn:bound1} and substitute back $\beta(t)=K+\alpha(t)$
	\begin{align}
	F(w(t+1)) &\leq  l_{t}(w(t+1))+\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t+1))-\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+(K+\alpha(t))h(w(t+1))\nonumber \\&-(K+\alpha(t))h(w(t)) +\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)}\\&\leq \sum_{t'=1}^{t}\tilde l_{t'}(w(t+1))-\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+(K+\alpha(t+1))h(w(t+1))\nonumber \\&-(K+\alpha(t))h(w(t)) +\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)}\label{eqn:temp52}
	\end{align}
	where \eqref{eqn:temp52} is due to $\alpha(t+1)\geq \alpha(t)$. Now, we use $\beta(t)=K+\alpha(t)$, multiply by $c(t+1)$ and rewrite
	\begin{align}
	c(t+1)F(w(t+1)) &\leq \sum_{t'=1}^{t}\tilde c(t+1)l_{t'}(w(t+1))-\sum_{t'=1}^{t-1}\tilde c(t)l_{t'}(w(t))+c(t+1)\beta(t+1)h(w(t+1))\nonumber \\&-c(t)\beta(t)h(w(t)) +c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)}\nonumber \\&-(c(t+1)-c(t))\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+\beta(t)h(w(t))\right]\label{eqn:temp53}
	\end{align}
	Sum from $t=1$ to $\tau -1$
	\begin{align}
	\sum_{t=2}^{\tau}c(t)F(w(t))\nonumber \leq & \sum_{t=1}^{\tau-1} c(\tau)\tilde l_{t}(w(\tau))+c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} \nonumber \\& +\sum_{t=1}^{\tau-1}(c(t)-c(t+1))\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+\beta(t)h(w(t))\right]
	\end{align}
	Let $\psi$ be the last two terms, i.e., 
	\begin{align}
	\psi =\sum_{t=1}^{\tau-1}(c(t)-c(t+1))\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+\beta(t)h(w(t))\right]
	\end{align}
	Using \cite{}Lemma 5
	\begin{align}
	\sum_{t=2}^{\tau}c(t)F(w(t))\nonumber \leq & \sum_{t=1}^{\tau-1} c(\tau)\tilde l_{t}(w^*)+c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi
	\end{align}
	By substituting \eqref{eqn:approx.first.order}
	\begin{align}
	\sum_{t=2}^{\tau}c(t)F(w(t))\nonumber  & \leq  \sum_{t=1}^{\tau-1} c(\tau) l_{t}(w^*)+ \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi \\ & \leq  \sum_{t=1}^{\tau-1} c(\tau) F(w^*)+ \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi \\ & = (\tau-1) c(\tau) F(w^*)+ \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi
	\end{align}
	Add and subtract terms
	\begin{align}
	\label{eqn:to.appendixE}\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]\nonumber  & \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}[c(\tau) - c(t)]  F(w^*)\nonumber \\ &  + \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi \\ & \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)\nonumber \\ &  + \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi
	\end{align}
	We take the expectation
	\begin{align}
	\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]\right]\nonumber  &  \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)\nonumber \\ & +c(\tau)\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1} \mathbb E [\langle q(t),w-w(t)\rangle]+\mathbb E[\langle r(t),w-w(t)\rangle] \nonumber \\ & +\sum_{t=1}^{\tau-1}c(t+1)\frac{\mathbb E [\|q(t)\|^2]+\mathbb [\|r(t)\|^2]}{4\alpha(t)} +\mathbb E[\psi]
	\end{align}
	We substitute 
	\begin{align}
	\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]\right]\nonumber  &  \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)\nonumber \\ & +c(\tau)\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)}  \nonumber \\ & +\sum_{t=1}^{\tau-1}\frac{c(t+1)}{4\alpha(t)} \left(\frac{\sigma^2}{b(t)}+\frac{K^2\epsilon^2}{\beta(t)^2}\right) +\mathbb E[\psi]
	\end{align}
	Let 
	\begin{align}
	\gamma = \max_{t \in \{1,\tau-1\}} \frac{c(t+1)}{b(t)}
	\end{align}
	and we rewrite
	\begin{align}
	\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]\right]\nonumber  &  \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)\nonumber \\ & +c(\tau)\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)}  \nonumber \\ & +\frac{\gamma \sigma^2}{4} \sum_{t=1}^{\tau-1}\frac{1}{\alpha(t)} +\frac{K^2\epsilon^2}{4}  \sum_{t=1}^{\tau-1} \frac{c(t+1)}{\alpha(t)\beta(t)^2} +\mathbb E[\psi]
	\end{align}
	Therefore, total regret by substituting above in \eqref{eqn:regret.first}
	\begin{align}
	\mathbb E[R]&   \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)+c(\tau)\beta(\tau)h(w(\tau)) \nonumber \\ & + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)} +\frac{\gamma \sigma^2}{4} \sum_{t=1}^{\tau-1}\frac{1}{\alpha(t)} +\frac{K^2\epsilon^2}{4}  \sum_{t=1}^{\tau-1} \frac{c(t+1)}{\alpha(t)\beta(t)^2} +\mathbb E[\psi] + L\epsilon \sum_{t=1}^{\tau} \frac{c(t)} {\beta( t)}\label{eqn:regret.second}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	Let $c_m = \max _t c(t)$. Then
	\begin{align}
	\mathbb E[R]&   \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)+c(\tau)\beta(\tau)h(w(\tau)) \nonumber \\ & + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)} +\frac{\gamma \sigma^2}{4} \sum_{t=1}^{\tau-1}\frac{1}{\alpha(t)} +\frac{K^2\epsilon^2c_m}{4}  \sum_{t=1}^{\tau-1} \frac{1}{\alpha(t)\beta(t)^2} +\mathbb E[\psi] + L\epsilon c_m \sum_{t=1}^{\tau} \frac{1} {\beta( t)}\label{eqn:regret.3}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	From Appendix 
	\begin{align}
	\mathbb E[R]&   \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)+c(\tau)\beta(\tau)h(w(\tau)) \nonumber \\ & + 2K D \epsilon \sqrt{\mu \tau }+\frac{2\gamma \sigma^2\sqrt{\mu \tau } }{4} +\frac{3K^2\epsilon^2c_m \mu ^{3/2}}{4}  + 2L\epsilon c_m\sqrt{\mu \tau } +\mathbb E[\psi]\label{eqn:regret.4}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	\begin{align}
	\mathbb E[R]&   \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)+c(\tau)\beta(\tau)h(w(\tau)) \nonumber \\ & +\frac{3K^2\epsilon^2c_m \mu ^{3/2}}{4} + \left(2K D \epsilon +\frac{\gamma \sigma^2 }{2}   + 2L\epsilon c_m\right)\sqrt{\mu \tau } +\mathbb E[\psi]\label{eqn:regret.5}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	Substituting Appendix 
	\begin{align}
	\mathbb E[R]&   \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}|c(\tau) - c(t)|  F(w^*)+c(\tau)\beta(\tau)h(w(\tau)) +\frac{3K^2\epsilon^2c_m \mu ^{3/2}}{4}  \nonumber \\ &+ \left(2K D \epsilon +\frac{\gamma \sigma^2 }{2}   + 2L\epsilon c_m\right)\sqrt{\mu \tau } + \delta \left( F(w^*)+K  +\sqrt{\frac{\tau }{\mu}}h(w^*)  +2 K D \epsilon\sqrt{\mu \tau }\right)\tau \label{eqn:regret.6}
	%\\ & = \mathbb E\left[\sum_{t=1}^{\tau} c(t)[ F(w(t))-F(w^*)]\right] + 3L\epsilon b \tau \sqrt{\mu \tau}
	\end{align}
	where $\delta=\max_{t \in \{1,\tau-1\}} |c(t)-c(t+1)|$.
	\subsection{Appendix B}
	Note that
	\begin{align}
	\mathbb E[f(w(t)),x_s(t)] =\mathbb E[F(w(t))]. 
	\end{align}
	Also we assume gradient and expectation operators commutes
	\begin{align}
	\mathbb E[\langle\nabla f(w(t)),x_s(t),w(t)\rangle] =\mathbb E[\langle F(w(t)),w(t)\rangle]. 
	\end{align}
	Now, we find $\mathbb E[\langle r(t),w^*-w(t)\rangle]$
	\begin{align}
	&\mathbb E[\langle r(t),w^*-w(t)\rangle] \\&= \mathbb E\left[\left\langle \frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w f(w_i(t),x_i(t,s)) - \frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w f(w(t),x_i(t,s)),w^*-w(t)\right\rangle\right] \\& =\mathbb E\left[\left\langle \frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w F(w_i(t)) - \frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w F(w(t)),w^*-w(t)\right\rangle\right]\\& =\frac{1}{b(t)} \sum_{i=1}^{n} b_i(t) \mathbb E\left[\left\langle \nabla_w F(w_i(t)) -\nabla_w F(w(t)),w^*-w(t)\right\rangle\right]\\&\leq \frac{1}{b(t)} \sum_{i=1}^{n} b_i(t) \mathbb E\left[ \| \nabla_w F(w_i(t)) -\nabla_w F(w(t))\|\|w^*-w(t)\|\right] \label{cauchy}
	\\&\leq \frac{1}{b(t)} \sum_{i=1}^{n} b_i(t) \mathbb E\left[K \|w_i(t) -w(t)\|D\right] \label{lip1}
	\end{align}
	where \eqref{cauchy} is due to Cauchy-Schwarz inequality and \eqref{lip1} due to this and this. Using \eqref{eqn:primary.bound}
	 \begin{align}
	 \mathbb E[\langle r(t),w^*-w(t)\rangle] &\leq \frac{1}{b(t)} \sum_{i=1}^{n} \frac{b_i(t) K D \epsilon}{\beta(t)}
	 \\& = \frac{K D \epsilon}{\beta(t)}
	 \end{align}
	Now we find $\mathbb E[\|r(t)\|^2]$.
	\begin{align}
	\mathbb E[\|r(t)\|^2]&=\mathbb E\left [\left\|\frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \nabla_w f(w_i(t),x_i(t,s)) -  \nabla_w f(w(t),x_i(t,s))\right\|^2\right]\\&\leq\mathbb E\left [\left(\frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \left\|\nabla_w f(w_i(t),x_i(t,s)) - \nabla_w f(w(t),x_i(t,s))\right\|\right)^2\right]\\&\leq\mathbb E\left [\left(\frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} K\left\|w_i(t) - w(t)\right\|\right)^2\right]\\&\leq\left(\frac{1}{b(t)} \sum_{i=1}^{n} \sum_{s=1}^{b_i(t)} \frac{K\epsilon}{\beta(t)}\right)^2
	\\ &= \frac{K^2\epsilon^2}{\beta(t)^2}
	\end{align}
	\subsection{Appendix B}
	We know $\beta(t)=K+\alpha(t)$. Let $\alpha(t)=\sqrt{\frac{t}{\mu}}$. The, we have
	\begin{align}
	\label{eqn:beta.bound}
	\sum_{t=1}^{\tau-1}\frac{1}{\beta(t)} \leq 2 \sqrt{\mu \tau}
	\end{align}
	\subsection{Appendix C}
	Let $\psi$ be the last two terms
	\begin{align}
	\psi &=\sum_{t=1}^{\tau-1}(c(t)-c(t+1))\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+\beta(t)h(w(t))\right]\\&\leq \sum_{t=1}^{\tau-1}|c(t)-c(t+1)|\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w(t))+\beta(t)h(w(t))\right]\\&\leq \sum_{t=1}^{\tau-1}\delta\left[\sum_{t'=1}^{t-1}\tilde l_{t'}(w^*)+\beta(t)h(w^*)\right]\\&= \sum_{t=1}^{\tau-1}\delta\left[\sum_{t'=1}^{t-1}l_{t'}(w^*)+\langle q(t'),w^*-w(t')\rangle+\langle r(t'),w^*-w(t')\rangle+\beta(t)h(w^*)\right]
	\\&\leq \sum_{t=1}^{\tau-1}\delta\left[F(w^*)+\beta(t)h(w^*)  +\sum_{t'=1}^{t-1}\langle q(t'),w^*-w(t')\rangle+\langle r(t'),w^*-w(t')\rangle\right]
	\\&\leq \tau\delta F(w^*)+\sum_{t=1}^{\tau-1}\delta\left[\beta(t)h(w^*)  +\sum_{t'=1}^{t-1}\langle q(t'),w^*-w(t')\rangle+\langle r(t'),w^*-w(t')\rangle\right]
	\end{align}
	where $\delta=\max_{t \in \{1,\tau-1\}} |c(t)-c(t+1)|$. We take the expectation over the data samples 
	\begin{align}
	\mathbb E[\psi] &\leq \mathbb e \left[\tau\delta F(w^*)+\sum_{t=1}^{\tau-1}\delta\left[\beta(t)h(w^*)  +\sum_{t'=1}^{t-1}\langle q(t'),w^*-w(t')\rangle+\langle r(t'),w^*-w(t')\rangle\right] \right] \\ &\leq \tau\delta F(w^*)+\sum_{t=1}^{\tau-1}\delta\left[\beta(t)h(w^*)  +\sum_{t'=1}^{t-1}\mathbb E \left[\langle q(t'),w^*-w(t')\rangle\right]+\mathbb E \left[\langle r(t'),w^*-w(t')\rangle\right]\right]\\ &\leq \tau\delta F(w^*)+\sum_{t=1}^{\tau-1}\delta\left[\beta(t)h(w^*)  +\sum_{t'=1}^{t-1}\frac{K D \epsilon}{\beta(t')}\right]
	\end{align}
	Using \eqref{eqn:beta.bound} we have
	\begin{align}
	\mathbb E[\psi] &\leq \tau\delta F(w^*)+\sum_{t=1}^{\tau-1}\delta\left[\left(K+\sqrt{\frac{t}{\mu}}\right)h(w^*)  +2 K D \epsilon\sqrt{\mu t}\right] \\ &\leq \delta \left( F(w^*)+K  +\sqrt{\frac{\tau }{\mu}}h(w^*)  +2 K D \epsilon\sqrt{\mu \tau }\right)\tau
	\end{align}
	\subsection{Appendix D}
	\begin{align}
	\sum_{t=1}^{\tau-1 }\frac{1}{\alpha(t) \beta(t)^2} &= \sum_{t=1}^{\tau-1 }\frac{1}{\alpha(t)(K+ \alpha(t)^2)}
	 \\ & \leq \sum_{t=1}^{\tau-1 }\frac{1}{ \alpha(t)^3}
	 \\ & = \mu^{3/2}\sum_{t=1}^{\tau-1 }t^{-3/2}
	 \\ & \leq \mu^{3/2}\left(1+\int_{{1}}^{\tau}t^{-3/2}dt\right)
	 \\ & \leq 3\mu^{3/2}
	\end{align}
	\subsection{Appendix E}
	We know 
	\begin{align}
	c(t)= \sum_{i=1}^{n} c_i(t) 
	\end{align}
	where $c_i(t)$ is the total number of gradients computed at the node $i$ at the $t$-th epoch. We assume $c_i(t)$ is independent and identically distributed according to some unknown processing time distribution. Let $\bar c = \mathbb E_p[c(t)]$, where expectation is over the processing time distribution. Similarly, let $1/\hat b = \mathbb E_p[1/b(t)]$. %Let the communication time at the $t$-th epoch is $T_c(t)$. As in our scheme, we fix the computation time to be $T$, there $c_i(t)$ is the number of gradients computed in $T+T_c(t)$ time by the node $i$. We assume, $c_i(t)$
	From \eqref{eqn:to.appendixE} we have
	\begin{align}
	\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]\nonumber  & \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}[c(\tau) - c(t)]  F(w^*)\nonumber \\ &  + \sum_{t=1}^{\tau-1}\langle q(t),w-w(t)\rangle+\langle r(t),w-w(t)\rangle \nonumber \\ & + c(\tau)\beta(\tau)h(w(\tau))+\sum_{t=1}^{\tau-1}c(t+1)\frac{\|q(t)\|^2+\|r(t)\|^2}{4\alpha(t)} +\psi
	\end{align}
	We take the expectation over data path condition on $c(t)$s and substitute 
	\begin{align}
	\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]|c(t)\right]\nonumber  &  \leq c(1)[F(w(1))-F(w^*)] + \sum_{t=1}^{\tau}[c(\tau) - c(t)]  F(w^*)\nonumber \\ & +c(\tau)\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)}  \nonumber \\ & +\sum_{t=1}^{\tau-1}\frac{c(t+1)}{4\alpha(t)} \left(\frac{\sigma^2}{b(t)}+\frac{K^2\epsilon^2}{\beta(t)^2}\right) +\mathbb E[\psi|c(t)]
	\end{align}
	Let $\alpha(t)=\sqrt{t/\bar c}$. Now we take expectation over the $c(t)$
	\begin{align}
	\mathbb E_p\left[\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]|c(t)\right]\right]\nonumber  &  \leq \bar c[F(w(1))-F(w^*)]  +\bar c\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)}  \nonumber \\ & +\sum_{t=1}^{\tau-1} \mathbb E_p\left[\frac{ c(t+1)}{4\alpha(t)} \left(\frac{\sigma^2}{b(t)}+\frac{K^2\epsilon^2}{\beta(t)^2}\right)\right] +\mathbb E_p[\mathbb E[\psi|c(t)]]
	\\&  = \bar c[F(w(1))-F(w^*)]  +\bar c\beta(\tau)h(w(\tau)) + \sum_{t=1}^{\tau-1}\frac{K D \epsilon}{\beta(t)}  \nonumber \\ & +\sum_{t=1}^{\tau-1} \frac{ \bar c}{4\alpha(t)} \left(\frac{\sigma^2}{\hat b}+\frac{K^2\epsilon^2}{\beta(t)^2}\right)
	\end{align}
	
	The last step is due to the fact that $c(t+1)$ and $b(t)$ are independent, i.e., two different epochs. Further $\mathbb E_p[\mathbb E[\psi|c(t)]]=0$. After further simplification with the use of Appendix B and D, 
	\begin{align}
	\mathbb E_p\left[\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]|c(t)\right]\right]\nonumber  &  \leq  \bar c[F(w(1))-F(w^*)  +\bar \beta(\tau)h(w(\tau))] + 2K D \epsilon \sqrt{\bar c \tau }  \nonumber \\ & +\frac{ \bar c\sigma^2 \sqrt{\bar c \tau} }{2\hat b}+\frac{3 K^2\epsilon^2\bar c^{5/2}}{4}
	\end{align}
	Taking the expectation over $c(t)$ of \eqref{eqn:regret.first}, we have
	\begin{align}
	\mathbb E_p [\mathbb E[R|c(t)]] &\leq  \mathbb E_p\left[\mathbb E\left[\sum_{t=1}^{\tau}c(t)[F(w(t))-F(w^*)]|c(t)\right]\right] + L\epsilon \sum_{t=1}^{\tau} \frac{\bar c} {\beta( t)} \\ & \leq  \bar c[F(w(1))-F(w^*)  +\bar \beta(\tau)h(w(\tau))] + 2K D \epsilon \sqrt{\bar c \tau }  \nonumber \\ & +\frac{ \bar c\sigma^2 \sqrt{\bar c \tau} }{2\hat b}+\frac{3 K^2\epsilon^2\bar c^{5/2}}{4}+ 2 L\epsilon \bar c \sqrt{\bar c \tau } 
	\end{align}
	We know 
	\begin{align}
	m=\sum_{t=1}^{\tau} c(t)
	\end{align}
	Let $\bar m = \mathbb E_p[m]$, thus $\bar m=\bar c \tau$. By substituting $\bar m$ and rearranging we get
	\begin{align}
	\mathbb E_p [\mathbb E[R|c(t)]] &\leq  \leq  \bar c[F(w(1))-F(w^*)  +\bar \beta(\tau)h(w(\tau))] +\frac{3 K^2\epsilon^2\bar c^{5/2}}{4}   \nonumber \\ & + \left(2K D \epsilon +\frac{ \bar c\sigma^2 }{2\hat b}+ 2 L\epsilon \bar c \right) \sqrt{\bar m } 
	\end{align}

